CHAM: action recognition using convolutional hierarchical attention model

Recently, the soft attention mechanism, which was originally proposed in language processing, has been applied in computer vision tasks like image captioning. This paper presents improvements to the soft attention model by combining a convolutional LSTM with a hierarchical system architecture to recognize action categories in videos. We call this model the Convolutional Hierarchical Attention Model (CHAM). The model applies a convolutional operation inside the LSTM cell and an attention map generation process to recognize actions. The hierarchical architecture of this model is able to explicitly reason on multi-granularities of action categories. The proposed architecture achieved improved results on three publicly available datasets: the UCF sports dataset, the Olympic sports dataset and the HMDB51 dataset.

==> Makefile <==
FILENAME = icip_paper
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf

# PAPERSIZE = a4
PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

pdf: main
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.7 \
		$(PS_FILE) $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

